SparCAssist: A Model Risk Assessment Assistant Based on Sparse Generated Counterfactuals

We introduce SparcAssist, a general-purpose risk assessment tool for the machine learning models trained for language tasks. It evaluates models' risk by inspecting their behavior on counterfactuals, namely out-of-distribution instances generated based on the given data instance. The counterfactuals are generated by replacing tokens in rational subsequences identified by ExPred, while the replacements are retrieved using HotFlip or Masked-Language-Model-based algorithms. The main purpose of our system is to help the human annotators to assess the model's risk on deployment. The counterfactual instances generated during the assessment are the by-product and can be used to train more robust NLP models in the future.

==> 01intro.tex <==
\section{Introduction}
\textcolor{red}{Attention: not finished!}
The text classification tasks are fundamental tasks in NLP (natural language processing) \cite{zhang2016rationale, yang2016hierarchical}. 
Along with the explosive development of artificial neural network technique, an extremely large family of well-performing models such as BERT\cite{bert}, BART\cite{lewis2019bart} and RoBERTa\cite{liu2019roberta} blossom. However, the fact that they functioning as black boxes hinges the researchers from inspecting such models on reasoning the predictions. To reveal the rationals behind the models' inference, several Post-hoc model interpretation approaches has been proposed. They are roughly categorized into 3 families: 1). feature-based, which highlights the most influential features globally while inference on a dataset such as \cite{expred}, \cite{lundberg2017unified} and \cite{ribiro2018anchors}; 2). instance-based, which selects similar instances or heuristic prototypes kin to each individual instance such as \cite{kim2016examples}, \cite{koh2019accuracy}
\begin{itemize}
    \item Posthoc counterfactual explanations help us in understanding why a blackbox model came up with a certain prediction
    \item  For humans to comprehend and contextualize these explanations they need to be `plausible'
    \item We demonstrate a system to generate plausible and meaningful counterfactual explanations with human-in-the-loop
    \item Using rationale text from ExPred and words selected by the HotFlip system, we suggest words to replace for humans which allows them to generate plausible and meaningful explanations.
    \item The goal is to generate a dataset of counterfactual explanations which are grammatically plausible and meaningful from human perspective.
    \item Insertion and deletion of words to generate counterfactual
    \item Beam search the replacement words with top-$k$ plausible words (grammatically).
\end{itemize}

Usefulness of human rational annotation: \cite{arous2021marta}\footnote{appendix: \url{https://exascale.info/assets/pdf/arous2020AAAI-sm.pdf}}

Importance of counterfactual in application: \cite{pmlr-v106-pfohl19a, hofler2005causal}

How to use counterfactual data: \cite{pmlr-v119-rieger20a}


\cite{hofler2005causal} provides an approach to identify causal relationship in the model inference using counterfactual instances

In causal inference study, counterfactual, or OOD (Out-Of- Distribution) instances, are usually referred to unobserved instances regarding a specific dataset, where some features are perturbed ("counter") from the 'real' instance drawn from the dataset ("factual"). They are useful to validate the robustness of the model under instance perturbation\cite{abbasnejad2020counterfactual}, or investigate model's decision boundary\cite{teney2020learning}. The concept "counterfactual" has been a well-defined representation of causality widely used in epidemiological and medical studies\cite{Hoefler2005}, financial\cite{yang2020generating} and NLP\cite{ross2020explaining}. In interpretable machine learning, the counterfactuals are also used to get better understanding by researching the effects of input features under limited perturbation\cite{wachter2017counterfactual, dandl2020multi}.

==> 02relworks.tex <==
\section{Related Works}
\label{sec:relatedworks}
In~\cite{zheng2021irrationality}, \citeauthor{zheng2021irrationality} investigate select-then-predict models such as works presented in ~\cite{lei-etal-2016-rationalizing, bastings-etal-2019-interpretable,expred}.
They argue that the select-and-predict models are essentially not interpretable from both philosophic and empirical aspects, while using generated counterfactuals could avoid this phenomenon.

\subsection{Counterfactual generation}
The counterfactual generation approaches can be categorized into two classes: human-annotation and machine-generation approaches.
Approaches like~\cite{mcdonnell2016relevant, kaushik2019learning} conduct user-study with crowd workers to get human-understandable counterfactual datasets.
But the data gathered from crowd workers suffer from high variance because of subjectivity and Rashomon effect~\cite{davis2015rashomon}.
Our \counterassist~restricts the users' choise and, therefore, assists to gather better counterfactual annotations easily.

The machine-generated approaches, on the other hand, provide systematic counterfactual generation models.

\hotflip~\cite{ebrahimi-etal-2018-hotflip} is one of the machine-based counterfactual generation approaches proposed by \citeauthor{ebrahimi-etal-2018-hotflip}.
It is an optimization-based way of generating counterfactuals.
The downside of the \hotflip~is its variable tokens are dense (every input token is variable), and the generated results are less meaningful.
We integrate \hotflip~as one of the counterfactual generation methods in \counterassist~and elucidate our implementation details in the following sections.


\citeauthor{wallace-etal-2020-imitation} provide an approach generating poisonous counterfactual instances to attack the translation system in ~\citet{wallace-etal-2020-imitation}.
More specifically, they propose a vicious counterfactual inputs generation approach, which optimizes the input sequences to predict the wrong but desired output.
% Their attack is over a distilled version~\cite{distilling_hinton} of the victim model.
% More specifically, they propose four different attacking counterfactuals that cause translating a token from input sequence into a specific target token in the output sequence (the \textbf{Targeted flips}) or lucid the translation model to ignore input content after some specific token (the \textbf{Universal Suffix Dropper}) and so on.
% Such vicious counterfactuals are constructed by optimizing the input sequences regarding the target output over a distilled version~\cite{distilling_hinton} of the victim model.
AutoPrompt~\cite{shin2020autoprompt} from \citeauthor{shin2020autoprompt} proposes a similar gradient-based approach.
% But the AutoPrompt is used to verify the ability of the modern pre-trained natural language encoders to learn the semantics of human languages.


\polyjuice~\cite{wu2021polyjuice} is yet another counterfactual generation approaches.
It leverages a prompt-based masked language model like Prompt-Tuning~\cite{DBLP:journals/corr/abs-2104-08691}, Prompt approach~\cite{prompt2019jiang} or P-Tuning~\cite{ptuning_liu} to generate counterfactuals.
They apply a blank-infill model~\cite{donahue-etal-2020-enabling} based on GPT-2~\cite{radford2019language} to predict the masked critical tokens in the input sequence.
Although results generated by \polyjuice~are more natural and meaningful, it does not restrict the density of variable tokens, either.
Not to mention its generation of counterfactuals is controlled by hand-craft prompts, which are limited and non-systematic.
We also apply the \mlm-based model for counterfactual generation and introduce the implementation in detail in the following sections.

\subsection{Human-in-the-loop ML model debugging}
As more stakeholders pay more attention to the model's correctness and rationale than only on the performance numbers, the HITL(Human-in-the-loop) machine learning~\cite{monarch2021human} has recently attracted more awareness.
The search engines themselves are typical examples leveraging HITL to optimize the performance of the machine learning models. As an example, the dissertation from~\citeauthor{avineshinformation}~\cite{avineshinformation} conclude how HITL approaches to improve search engine and envision the use of interactive NLP models.
While model attacking approaches~\cite{misra2019black, wallace-etal-2020-imitation} expose model's deployment risk by trying to lucid them to predict unexpected results, HITL-ML model debuggers introduce human control and make the models \emph{right for the right reason}.
A number of HITL model debugging approaches has also been proposed~\cite{10.1162/tacl_a_00440, DBLP:journals/corr/abs-2010-04987}.
Along with these academic researches, the HITL-ML model debugging tools, like SageMaker\footnote{\url{https://aws.amazon.com/cn/sagemaker/}} provided by Amazon, have also taken a gradually large share of the market.

% \cite{pfohl2019counterfactual} is yet another generative counterfactual producer that leverages VAE \cite{kingma2014autoencoding} to generate counterfactuals.
% \citeauthor{pfohl2019counterfactual} also suggest using equalized odd \cite{hardt2016equality} to assess the robustness of a model when presented with different counterfactual instances.


% \cite{kim-etal-2020-interpretation} and \cite{harbecke-alt-2020-considering} are two counterfactual generation approaches based on IM (input marginalization).
% However, \citeauthor{pham2021double} point it out that the IM does not always perform better than leave-one-out approaches like\cite{li2016understanding,NIPS2017_7062} despite being \~5 to 10x more computationally expensive.
 
% The work from \citeauthor{gardner2020evaluating} (\cite{gardner2020evaluating}) summarizes three possible contrasting generation methods\cite{dua2019drop, suhr2018corpus,suhr2018corpus,nivre2016universal} to generate contrastive sets.
% Their work aims mainly to outline local decision boundaries of an NLP model, therefore their contrastive set might be far distant from the original instance and are not counterfactuals we mentioned here.

% The work from \citeauthor{gardner2020evaluating} (\cite{gardner2020evaluating}) summarizes three possible contrasting generation methods\cite{dua2019drop, suhr2018corpus}, NLVR2\cite{suhr2018corpus}, and UD Parsing\cite{nivre2016universal} to generate contrastive sets for 10 datasets including NLVR2, IMDb sentiment analysis\cite{maas2011learning}, and so on.
% Their work aims mainly to outline local decision boundaries of an NLP model, therefore their contrastive set might be far distant from the original instance and are not counterfactuals we mentioned here.


==> _04approache_backup.tex <==
% % \section{Approach}
% % In this paper, we provide three different approaches to generate counterfactual instances confined to the rules presented in the previous section.
% If otherwise specified, we assume all the models used for the inference are pre-trained, i.
% e.
% we generate counterfactuals for post-interpretation.



% % \subsection{Invariant Length Direct Replacement}

% % \textcolor{red}{we have actually three possible possible tasks regarding the counterfactual:

% % 1.
% train a high-performance model sustaining the bombardier of the counterfactual.
% In a way the model's representation of the original and the non-evident counterfactuals are near to each other, while the evident counterfactuals are embedded far from the original one.
% Here the counterfactuals can be either crafted by hand or selected by another model.


% % 2.
% Build a counterfactual generating template, that generates counterfactuals satisfying the requirement mentioned above for its corresponding pre-trained model.
% Then apply this counterfactual-generation framework to the pre-trained model.
% There 5 possible outcomes: \{evident counterfactual, non-evident counterfactual\} * \{semantic variant, stable\} and impure counterfactual.
% Out of these four outcomes, a) evident counterfactual + semantic variant and b) non-evident counterfactual + semantic invariant are the \textit{normal} states and nothing specific need to be paid attention.
% The rests indicates either bugs in the language representation model or deficiencies in the counterfactual generation framework.
% The outcome c) evident counterfactual + semantic stable indicates that although the explanation model catches this evidence, this part of evidence does not contribute much to the sentence meaning, while the d) non-evident counterfactual + semantic variance indicates the model unduly upweights this non-evident token.
% The final situation, impure counterfactual means the perturbed terms including both evidence and non-evidence terms.
% This indicates the counterfactual generation framework is not well trained.


% % 3.
% The deep learning models are essentially data-driven programs.
% Their debug can only be done by acquiring more specific dataset.
% The uncommon behavior mentioned in 2 actually provides the new training data, based on which one can  }
% % For most NLP tasks, a good language representation model is necessary.
% Formally speaking, a representation model $h$ converts the original input to a (bunch of) vector(s) in the hidden space $h(x)$.
% Our second approach is is based on such hypothesis, that the hidden representation of the original instance $h(x)$ and of the counterfactual instance $h(x^c)$ should be the same, or they should locate as near as possible, if the semantic meaning stays the same regarding the NLP task.
% For instance consider in a semantic analysis task, $h$ is its language representation model.
% For the original instance $x$: \textit{This movie is good.
% }, one can construct its two counterfactuals $x^c_1$: \textit{This movie are good.
% } and $x^c_2$: \textit{This movie is bad.
% }.
% Albeit its syntax error, $x_c_2$ states the same fact that the movie is to be complimented, and its hidden representations should be the same or locate not far from $h(x)$.
% The $x^c_2$, however, is a critic against the movie thence $h(x^c_2)$ should be away from $h(x)$.
% Such difference of the hidden representation divides all counterfactuals into two categories: semantic stable and semantic variant ones.


% % Furthermore, based on the position of the fluctuation, we can also split counterfactuals flipping the tokens in evidence only and the ones 
% % At first, we train the first-phase of the \expred~interpretable model.
% This phase 1 model is an MTL (Multi-Task-Learning) model, because it emits both the classification task prediction and the extracative explanation for the task as its two simultaneous outputs.
% The extracted explanations should satisfy both sufficiency and comprehensiveness introduced in \cite{deyoung-etal-2020-eraser}.
% This is to say, the information needed for the classification should be contained in and only be contained in the explanations.
%  so that its output to generate rationale annotation
% % 2.
% Fine-tune a normal BERT for the task on full sequential input (no rational mask)
% % 3.
% Make a snapshot of the current word embeddings
% % 4.
% Freeze the normal BERT parameter and the embedding of the non-rationale tokens, let loose of the embedding of the rationale tokens, fine-fine tune the representation of the rationale tokens.
% During the training we don't care whether the representation of the token represents embeddings in the snapshot.

% % 5.
% After the post-fine-tuning, retrieve the nearest neighbour of the continuous representation from the snapshot.


% % This is inspired by p-tuning \cite{ptuning_liu} and prompt-tuning \cite{prompt_tuning_lseter}, where their prompt of generating new sequences are continuous in the embedding space.
% This approach assures the generated counterfactual instance is the same length of the original input.


% % \subsection{Controllable Generation without length restriction}
% % The beginning of this approach the same as the privious one, i.
% e.
% training the phase 1 model of \expred .


% % After the rationale identifier identifies the rationales, modify the input sequence to add start and end marks of the rationales.
% Such as:

% % This movie is [BOR] fascinating [EOR].


% % where the [BOR] stands for "the beginning of the rationale" and the [EOR] stands for "the ends with the rationales".


% % Use an auto-regression model (e.
% g.
% multi-layer LSTM) as the classification model.
% Train the classification model on the modified dataset in the following manner:

% % 1.
% The input combines the classification and the sequence
% % 2.
% The output tries to predict the next token given current tokens and the classification.


% % After training the classification model, flip all classifications input, keep the non-rationale input sequence unchanged.
% Whenever there is a [BOR] in the input, replace the consequential input with the predicted counterfactual rationales, until the counterfactual generator generates an [EOR].
% Then switch back to the original non-rationale input starts with its [EOR]

% % during training:

% % input: [NEG] This movie is [BOR] boring [EOR].
% I was almost asleep.
% [EOS]

% % output: This movie is [BOR] boring [EOR].
% I was almost asleep.
% [EOS][EOS]

% % Notice that the output should predict 'movie' when the input takes "[NEG]" and "This".


% % during inference:

% % input: [POS] This movie is [BOR] super fascinating [EOR].
% I was almost asleep.
% [EOS]

% % output: This movie is [BOR] super fascinating [EOR].
% I was almost asleep.
% [EOS]

% % The 'super' is predicted after inputting '[POS] This movie is [BOR]'.
% Eventually the counterfactual generator generates three tokens: 'super fascinating [EOR]' and they replaced the 'boring [EOR]' and serve as the input.
% After the outputting the '[EOR]', we switch back the input source to the original input.


% % This approach is inspired by the prompting strategy in inspecting the knowledge encoded in language models like in GPT-2\cite{radford2019language}, GPT-3\cite{gpt3}, auto-prompt\cite{autoprompt} and \cite{prompt2019jiang}.
% In these approaches, models are not even fine-tuned but provided with some additional prompts after the input.
% For example the prompt can be 'This movie is' if one would like to express the sentiment of the review in the statement, or can be 'In short, this story tells that' for document summarizing.
% Then one can let loose and let the model to generate freely after the prompt


% % At first, the end users are presented by the web app with a randomly selected document together with its corresponding query from the dataset (1).
% The detail of the dataset we used will be presented in the following section.
% Without losing the generality, we take the following query-document pairs as our running example:
% % \begin{itemize}
% %     \item \textbf{Query}: \textit{What is the sentiment of this review?}
% %     \item \textbf{Doc}: \textit{This movie is fantastic.
% I am always fancy in the masterpieces of Kubrick's.
% }
% % \end{itemize}

% % \textcolor{red}{based on pretrained RoBERTa\cite{DBLP:journals/corr/abs-1907-11692} model.
% The pre-training weights are provided by the Huggingface\footnote{\url{https://huggingface.
% co/docs/transformers/main_classes/pipelines#transformers.
% FillMaskPipeline}}}

% % Then the users are asked to select one sentence from the given document, say the first sentence \textit{This movie is fantastic.
% }, to inspect \textbf{(2)}.
% The application then passes the selected sentence together with the query to the \expred to get the initial explanation and prediction \textbf{(3)}.
% The initial explanation and prediction are presented to both the end user and automatic counterfactuals generators \textbf{(4)}.
% The machine generated rationales are presented highlighted to the user While the counterfactual generators, will try to alternate the final prediction of \expred by replacing one or more words from rationale sub-sequence  (perturb).
% Such perturbed sentences are our automatically generated counterfactual instances of the given sentence.
% They are presented to the users as examples of possible perturbations \textbf{(5)}.
% The users are asked to finish two tasks given the examples: a) to evaluate the counterfactuals and b) to generate their own counterfactuals.
% For evaluation, one need to tell whether the counterfactual generators exposes the model bias by flipping the contextual words, or they indeed flip the critical tokens \textcolor{red}{need to formally define the irrelevant, contextual and critical tokens in section problem statement}.
% For either case, the user is encouraged to provide his own counterfactual, either to expose the bias one step further (alternating the prediction by substituting the contextual words) or to indicate the critical words by replacing them with their antonyms.


% % \textcolor{red}{Need screenshots of the demo with different usecases}

==> _05implement.tex <==
% \section{Experiments Setup and Evaluation Methods}
% \subsection{Experimental setup:}
% \begin{itemize}
%     \item Restrict the demo to 10 documents? and collect feedback.
%     \item Every sentence containing a bold word.
%     \item Give feedback on grammatical clarity ($1-5$) and human plausibility ($1-5$).
%     \item How long it took for the user to find the best custom mask for the plausible counterfactual or it was found within 5 flips.
%     \item Average scores for the clarity and plausibility.
%     \item Repeat this for ExPred and custom setup?
% \end{itemize}

% \textcolor{red}{Collect some data internally and analyze the scores for the counterfactual}





==> _06results.tex <==
% \section{Results Analysis}

==> _08ack.tex <==
\begin{acks}

\end{acks}
